Multi-Object Grasping -- Types and Taxonomy

This paper proposes 12 multi-object grasps (MOGs) types from a human and robot grasping data set. The grasp types are then analyzed and organized into a MOG taxonomy. This paper first presents three MOG data collection setups: a human finger tracking setup for multi-object grasping demonstrations, a real system with Barretthand, UR5e arm, and a MOG algorithm, a simulation system with the same settings as the real system. Then the paper describes a novel stochastic grasping routine designed based on a biased random walk to explore the robotic hand's configuration space for feasible MOGs. Based on observations in both the human demonstrations and robotic MOG solutions, this paper proposes 12 MOG types in two groups: shape-based types and function-based types. The new MOG types are compared using six characteristics and then compiled into a taxonomy. This paper then introduces the observed MOG type combinations and shows examples of 16 different combinations.

==> backup.tex <==
//in-hand manipulation
Dexterous manipulation has been an active area of research for decades (bicchi2000hands; fearing1986implementing; ma2011dexterity; Okamura et al., 2000; rus1999hand). Many different approaches and strategies have been proposed over the years. This includes rolling (Bicchi and Sorrentino, 1995; Cherif and Gupta, 1999; Doulgeri and Droukas, 2013; Han et al., 1997; Han and Trinkle, 1998), sliding (Cherif and Gupta, 1999; Shi et al., 2017), finger gaiting (Han and Trinkle, 1998), finger tracking (Rus, 1992), pushing (Dafle and Rodriguez, 2017), and re-grasping (Dafle et al., 2014; Tournassoud et al., 1987). For some hand types, strategies such as pivoting (Aiyama et al., 1993), tilting (Erdmann and Mason, 1988), tumbling (Sawasaki and Inoue, 1991), tapping (Huang and Mason, 2000), two-point manipulatio

Bicchi A. (2000) Hands for dexterous manipulation and robust grasping: A difficult road toward simplicity. IEEE Transac- tions on Robotics and Automation 16(6): 652–662.
Fearing RS (1986) Implementing a force strategy for object re- orientation. In: Proceedings of the 1986 IEEE International Conference on Robotics and Automation, San Francisco, CA, 7–10 April 1986, pp. 96–102.
Ma RR and Dollar AM (2011) On dexterity and dexterous manip- ulation. In: 15th International Conference on Advanced Robotics: New Boundaries for Robotics (ICAR 2011), Tallinn, Estonia, 20–23 June 2011, pp. 1–7.
Okamura AM, Smaby N and Cutkosky MR (2000) An overview of dexterous manipulation. In: Proceedings of the 2000 IEEE International Conference on Robotics and Automation (ICRA 2000), San Francisco, CA, 24–28 April 2000, pp. 255–262.
Rus D. (1999) In-hand dexterous manipulation of piecewise- smooth 3-D objects. The International Journal of Robotics Research 18(4): 355–381.
Bicchi A and Sorrentino R. (1995) Dexterous manipulation through rolling. In: Proceedings of the 1995 International Conference on Robotics and Automation, Nagoya, Aichi, Japan, 21–27 May 1995, pp. 452–457.
Cherif M and Gupta KK. (1999) Planning quasi-static fingertip manipulations for reconfiguring objects. IEEE Transactions Robotics and Automation 15(5): 837–848.
Doulgeri Z and Droukas L (2013) On rolling contact motion by robotic fingers via prescribed performance control. In: 2013 IEEE International Conference on Robotics and Automation, Karlsruhe, Germany, 6–10 May 2013, pp. 3976–3981.
Han L, Guan Y, Li ZX, Qi S and Trinkle JC. (1997) Dextrous manipulation with rolling contacts. In: Proceedings of the 1997 IEEE International Conference on Robotics and Automation, Albuquerque, NM, 20–25 April 1997, pp. 992–997.
Cherif M and Gupta KK. (1999) Planning quasi-static fingertip manipulations for reconfiguring objects. IEEE Transactions Robotics and Automation 15(5): 837–848.
Shi J, Woodruff JZ, Umbanhowar PB and Lynch K. (2017) Dynamic in-hand sliding manipulation. IEEE Transactions on Robotics 33(4): 778–795.
Han L and Trinkle JC. (1998) Dextrous manipulation by rolling and finger gaiting. In: Proceedings of the IEEE International Conference on Robotics and Automation (ICRA-98), Leuven, Belgium, 16–20 May 1998, pp. 730–735.
Rus D (1992) Dexterous rotations of polyhedra. In: Proceedings of the 1992 IEEE International Conference on Robotics and Automation, Nice, France, 12–14 May 1992, pp. 2758–2763.
Dafle NC and Rodriguez A. (2017) Sampling-based planning of in-hand manipulation with external pushes. CoRR abs/ 1707.00318.
Dafle NC, Rodriguez A, Paolini R, et al. (2014) Extrinsic dexter- ity: In-hand manipulation with external forces. In: 2014 IEEE International Conference on Robotics and Automation (ICRA 2014), Hong Kong, China, 31 May–7 June 2014, pp. 1578– 1585.
Tournassoud P, Lozano-Pe ́rez T and Mazer E. (1987) Regrasping. In: Proceedings of the 1987 IEEE International Conference on Robotics and Automation, Raleigh, NC, 31 March–3 April 1987, pp. 1924–1928.
Aiyama Y, Inaba M and Inoue H (1993) Pivoting: A new method of graspless manipulation of object by robot fingers. In: Pro- ceedings of 1993 IEEE/RSJ International Conference on Intel- ligent Robots and Systems (IROS 1993), Tokyo, Japan, 26–30 July 1993, pp. 136–143.
Erdmann MA and Mason MT. (1988) An exploration of sensorless manipulation. IEEE Journal of Robotics and Automation 4(4): 369–379.
Sawasaki N and Inoue H. (1991) Tumbling objects using a multi- fingered robot. Journal of the Robotics Society of Japan 9(5): 560–571.
Huang WH and Mason MT. (2000) Mechanics, planning, and control for tapping. The International Journal of Robotics Research 19(10): 883–894.


\begin{table}[h!]
\begin{center}
\begin{tabular}{ |p {1.5cm}|p {2.5cm}|c| } 
 \hline
 \multicolumn{3}{c}{Hand Shape}\\ \hline
 finger-palm clip & One finger is pressing toward the palm with one or more objects in between.
 &  \includegraphics[width=0.4\columnwidth]{figures/square-pyr-2-15.jpg} \\ \hline
finger-finger clip & One finger is pressing toward the palm with one or more objects in between.
 &  \includegraphics[width=0.4\columnwidth]{figures/square-pyr-2-15.jpg} \\ \hline
 fingertip-fingertip pinch & Two finger & \includegraphics[width=0.4\columnwidth]{figures/cub-3-14.jpg} \\ \hline
 
 lateral pinch & A finger presses objects on the side of another finger.  & \includegraphics[width=0.4\columnwidth]{figures/tri-46.jpg} \\ \hline
 
 scissors & Objects are held by the sides of two fingers. & \includegraphics[width=0.4\columnwidth]{figures/cyl-5-81-l.jpg} \\ \hline
 cup  & Fingers form a cup that holds objects in.   & \includegraphics[width=0.4\columnwidth]{figures/pris-97-b.jpg} \\ \hline 

\end{tabular}
\caption{Grasp types based on hand shapes, interaction, and ???}
\end{center}
\end{table}

\begin{table}[h!]
\begin{center}
\begin{tabular}{ |p {1.5cm}|p {2.5cm}|c| } 
 \hline
 \multicolumn{2}{c}{Type (Continue)}\\ \hline \hline
 
funnel & funnel& \includegraphics[width=0.4\columnwidth]{figures/pris-7-30-f.jpg} \\ \hline

 cylindrical*  & cylindri & \includegraphics[width=0.4\columnwidth]{figures/cyl-7-44-bak.jpg} \\ \hline
 
 Track  & Two fingers act as track rails & \includegraphics[width=0.4\columnwidth]{figures/ball-3-89-3.jpg} \\ \hline
 
\end{tabular}
\end{center}
\end{table}

\begin{table}[h!]
\begin{center}
\begin{tabular}{ |p {1.5cm}|p {2.5cm}|c| } 
 \hline
 \multicolumn{2}{c}{combined types (Examples)}\\ \hline \hline
two or more finger-palm clips & Two or more fingers are pressing toward the palm with one or more objects in between & \includegraphics[width=0.4\columnwidth]{figures/block-3-60.jpg} \\ \hline
Clip \& pinch & &  \includegraphics[width=0.4\columnwidth]{figures/ball-2-64-0.jpg} \\ \hline
  Clip \& cup & Fingers form a cup that holds objects in. Another finger form a clip shape and cover the open of the ``cup''.  & \includegraphics[width=0.4\columnwidth]{figures/ball-4-151.jpg} \\ \hline

\end{tabular}
\end{center}
\end{table}

\begin{table}[h!]
\begin{center}
\begin{tabular}{ |p {1.5cm}|p {2.5cm}|c| } 
 \hline
 \multicolumn{3}{c}{Human grasp types}\\ \hline
 finger-palm clip & One finger is pressing toward the palm with one or more objects in between.
 &  \includegraphics[width=0.4\columnwidth]{figures/image002.png} \\ \hline
 fingertip-fingertip pinch & Two finger & \includegraphics[width=0.4\columnwidth]{figures/image001.png} \\ \hline
scissors & Objects are held by the sides of two fingers & \includegraphics[width=0.4\columnwidth]{figures/image007.png} \\ \hline
 & & \includegraphics[width=0.4\columnwidth]{figures/image018.png} \\ \hline
 funnel & funnel& \includegraphics[width=0.4\columnwidth]{figures/image047.png} \\ \hline
  & & \includegraphics[width=0.4\columnwidth]{figures/image080.png} \\ \hline
  & & \includegraphics[width=0.4\columnwidth]{figures/image090.png} \\ \hline
  lateral pinch & A finger presses objects on the side of another finger.  & \includegraphics[width=0.4\columnwidth]{figures/image192.png} \\ \hline

\end{tabular}
\end{center}
\end{table}

\begin{table}[h!]
\begin{center}
\begin{tabular}{ |p {1.5cm}|p {2.5cm}|c| } 
 \hline
 \multicolumn{3}{c}{Human grasp types}\\ \hline
 & & \includegraphics[width=0.4\columnwidth]{figures/180.JPG} \\ \hline
 & & \includegraphics[width=0.4\columnwidth]{figures/182.JPG} \\ \hline
 & & \includegraphics[width=0.4\columnwidth]{figures/189.JPG} \\ \hline

\end{tabular}
\end{center}
\end{table}

